Quantum Laurent positivity in rank three

We prove Laurent positivity for skew-symmetrizable quantum cluster algebras of rank three, with arbitrary integral compatible quantizations and invertible frozen variables. The proof uses mutation-acyclic positivity from a companion manuscript.

==> _backup_E1E2E3_20260925_014803/bibliography_rank3.tex <==
\begin{thebibliography}{99}
\raggedright
\bibitem{BZ} A. Berenstein and A. Zelevinsky, \emph{Quantum cluster algebras}, \href{https://arxiv.org/abs/math/0404446v2}{arXiv:math/0404446v2} (2004).
\bibitem{Davison} B. Davison, \emph{Positivity for quantum cluster algebras}, \href{https://arxiv.org/abs/1601.07918v6}{arXiv:1601.07918v6} (2017).
\bibitem{FZ1} S. Fomin and A. Zelevinsky, \emph{Cluster algebras I: Foundations}, \href{https://arxiv.org/abs/math/0104151v1}{arXiv:math/0104151v1} (2001).
\bibitem{GHKK} M. Gross, P. Hacking, S. Keel and M. Kontsevich, \emph{Canonical bases for cluster algebras}, \href{https://arxiv.org/abs/1411.1394v2}{arXiv:1411.1394v2} (2016).
\bibitem{LS3} K. Lee and R. Schiffler, \emph{Positivity for cluster algebras of rank 3}, Publ. Res. Inst. Math. Sci. \textbf{49} (2013), no. 3, 601--649. \href{https://arxiv.org/abs/1205.5466v2}{arXiv:1205.5466v2}. \href{https://doi.org/10.4171/PRIMS/114}{doi:10.4171/PRIMS/114}.
\bibitem{LS} K. Lee and R. Schiffler, \emph{Positivity for cluster algebras}, Ann. of Math. \textbf{182} (2015), 73--125. \href{https://arxiv.org/abs/1306.2415v3}{arXiv:1306.2415v3}.
\bibitem{MA} Q. Tang, \emph{Quantum Laurent positivity for mutation-acyclic cluster algebras}, unpublished manuscript, 2026.
\end{thebibliography}

